DAWT: Densely Annotated Wikipedia Texts across multiple languages

In this work, we open up the DAWT dataset - Densely Annotated Wikipedia Texts across multiple languages. The annotations include labeled text mentions mapping to entities (represented by their Freebase machine ids) as well as the type of the entity. The data set contains total of 13.6M articles, 5.0B tokens, 13.8M mention entity co-occurrences. DAWT contains 4.8 times more anchor text to entity links than originally present in the Wikipedia markup. Moreover, it spans several languages including English, Spanish, Italian, German, French and Arabic. We also present the methodology used to generate the dataset which enriches Wikipedia markup in order to increase number of links. In addition to the main dataset, we open up several derived datasets including mention entity co-occurrence counts and entity embeddings, as well as mappings between Freebase ids and Wikidata item ids. We also discuss two applications of these datasets and hope that opening them up would prove useful for the Natural Language Processing and Information Retrieval communities, as well as facilitate multi-lingual research.

==> texfiles/wiki-markup_acknowledgements.tex <==
We thank ...

==> texfiles/wiki-markup_derivation.tex <==
\subsection{Methodology}
\label{sec:methodology}

\subsubsection{Unifying Entity Id Space}

\subsubsection{Candidate Dictionary}

The initial mappings of entity to possible aliases we call candidate dictionary.
Here the primary task is not to derive alias entity probabilities or any numerical association between them as it may be
hard task, but it's to capture  all reasonable alias for a given entity.
Candidate dictionary overview is shown in Figure \ref{fig:vanilla_dictionary}.
The candidate dictionary was derived by merging Wikipedia: titles, direct anchor texts, and redirects;
Freebase: aliases, and also known as; Wikidata: aliases; and English Wikiconcepts: anchor texts.
Merge is done for all available languages from each resource.
Due to nature of the sources and fact that any of them are manually edited and anchored.
Candidate lists had to go under alias alignment process, in which entities that map to many
aliases and have been pruned out of outlier aliases.
As a semantic alignment metrics of two phrases we used combination of:
Jaccard similarity (both token and 3-gram character), edit distance (token and character), and
largest common subsequent. The metrics were averaged. Then for each candidate in the list we calculated
average alignment against all  the other candidates. As final step we remove all candidates if any, with lowest alignment scores.
For example:

Example of some of unaligned entities in original mapping for the entity USA for examples were
"our" as in wiki some text may achor "our" linked to USA when while referring to it.
Other such examples are :  "pro Union", "New", "American Country Music Singer" etc as they do not allign well
with rest of the candiate aliases eg. "u.s. of america", "u.s.a", "USA" "United states", "America's",
"The United States Of America", etc. Alignment between two strings was calculates ax mixture of
different string similarity metrics (edit distance, longest common substring, and character n-gram and token
based Jaccard Similarity). Finally alignment with rest of the dictionary set was calculated as average,
alignemnt of given entity against all other entites within the candidate set. We keep aliases with allignment value
with more than $0.1$ and consider only top 200 aligned aliases at most.




% select language, count(*) as cnt, sum(size(aliases)), sum(size(positive_alias_alignment))
% from tmp_entity_aliases_aligned group by language order by cnt desc limit 100;
%
% en	20310759	40820229	36690410
% fr	4539216	8857454	7970078
% de	4287847	9731459	8655750
% es	3977903	6435256	5998427
% ru	3712321	8097801	7245944
% it	3711906	6158490	5678011
% ja	3466880	5319376	5023877
% zh	3281773	4101427	3983004
% nl	2870347	4307472	4062856
% sv	2814500	4532722	4188055
% pl	2654746	5062505	4665467
% pt	2574920	4156157	3862302
% uk	1855802	3116293	2933317
% no	1419113	1838619	1789532
% id	1391659	1652520	1628363
% ar	1088929	1583593	1502522
% sr	873122	1583136	1422201
% zh-tw	426914	623536	623447
% zh-cn	426914	427036	427036
% vi	415885	541478	519763
% zh-hant	386977	424320	421194
% fa	352662	439550	436529
% ca	324445	907431	788426
% ko	293782	386845	381525
% ro	292347	356550	353971
% fi	284802	512655	473040
% tr	249219	290693	289506
% hu	248079	292735	291579
% cs	228817	267528	267050
% ms	185806	199449	199249
% hi	173563	226138	222301
% sk	157440	188323	187881
% da	155001	188804	188126
% bg	146846	171877	171349
% hr	129602	186876	183249


\subsubsection{Wikilinkification}



Vanilla Alias To Candidate Entities Dictionary how it was generated.


\begin{figure}[t]
\centering
\includegraphics[width=85mm]{figure/pdf/wiki_vanilla_dictionary.pdf}
\caption{Candidate Dictionary Generation Overview}
\label{fig:vanilla_dictionary}
\end{figure}



Below this line who knows if we need ?

In our setup we do not deploy sophisticated algorithms in order to create label data set, but rather constrain our
problem in such  manner that creating labels is trivial, and highly accurate.
For example having a task of entity linking on a sentence {\it 'The quick brown fox jumps over the lazy dog'} where possible
entity pool includes $ E_{hard} = { fox\_tv,  fox\_animal, hot\_dog, dog\_animal, dog\_symbolism} $ vs.
$ E_{easy} = {fox\_animal, dog\_animal} $ one may have to deploy totally different approaches. In a past due to
increased hardness of problem with as the pool of entities grows the disambiguation becomes  more tricky.

As a basic for our data set we use Wiki Markup, and anchor text that is linking directly to the entity wiki pages.
This set out of box has high precision, but very low recall as only ast most one mention of entity within article will
link to it's wikipedia page. This is the methodology and building blocks of the system:


\subsubsection{Wikipedia Article To Entity Mapping}

As the entity identifier we used Freebase $machineId$'s. Primarily as Freebas entities have been already already
linked across different languages by Linking to their language specific Wikipedia articles.
In order to build comprehensive mapping of the Freebase entity $machineId$'s to the Wikipedia articles,
we used:
\begin{enumerate}
   \item Wikipedia redirects within same language.
   \item Freebase links to the language specific Wiki pages.
\end{enumerate}

First we self join Wikipedia redirects to derive all of the article to article mappings for all articles
being part of same transient closure. Latter table was joined with entity to wiki article mapping derived from the
Freebase. Statistic for this mapping across different languages are shown in Table \ref{table:wiki_article_to_entity}.



TODO(nemanja) - is this needed now ?
\begin{table}[htbp]
\begin{center}
    \begin{tabular}{ | l | l | l | }
    \hline
    Language & Alias Count & Entity Count \\ \hline
    en & 5,004,647 & 1,253,940 \\ \hline
    es & 492,943   & 370,345 \\ \hline
    it & 401,958   & 152,298 \\ \hline
    de & 1,129,574 & 370,345 \\ \hline
    fr & 1,014,194 & 375,051 \\ \hline
    ar & 210,285   & 202,733 \\
    \hline
    \end{tabular}
\end{center}


\caption{Text Alias To Entity Mapping Stats}
\label{table:wiki_article_to_entity}
\end{table}

\subsubsection{Entity to Aliases Mapping}

Alias is text free form in which we may expect entity to appear
(eg. entity '018w8'  could map to  \{ 'Barack Obama', 'President Obama', 'Obama', ... \}.
We generate such mappings per language by aggregating frequencies of following:

\begin{enumerate}
  \item Entity to text based on Freebase predicates including: type object name, common topic alias, and rdf schema label.
  \item Entity to Wikipedia Article Title (including all applicable redirects)
  \item Entity to anchor text of Wikipedia Markup linking to the entity's wiki article
\end{enumerate}


Then from alias to all potential enties mapping and their observed frequencies we pick only top 5 most frequently observed
entities for a given alias.



\subsubsection{Entity Cooccurrence Frequencies}

We also use entity coocurance derived from Wikipedia Markup links to articles. Two entities are assumed to cooccur
within article only if links to their page are not separated by more than 10 tokens, ignoring the sentence or paragraph
breaks. Empirically this seem to work. The coocurance is later used to exapand list of potential entities that we may
expect to observe on a page. For each entity we considered only entities that co-occur 3 or more times, and we limit
number co-occuring entities to 50 most frequent ones.

\subsubsection{Data Set Derivation}

While not geting in to the details of the implementation we se standard Lucene Tokenizer as it supports well
range of languages. Both markup text and aliases were tokenized in the same way. When performing alias annotation we
iterate all non labeled tokens sequentially and match sequences of 1 to 6 shingles long against alias to entity
mappings. The entity belonging to longest token seqence is selected if any. At this point we might have multiple
entity candidates, or none. In case of none we resume to the next token and repeat. In case of multiple
entities we select one that satisfies first condition in following order:

\begin{enumerate}
  \item Select entity which originally appeared on the page.
  \item Select entity with hightest cooccurance with other entities originally anchored
\end{enumerate}


\begin{algorithm}
\caption{Entity To Wiki Article}\label{euclid}
\begin{algorithmic}[1]

\Procedure{Euclid}{$W,Ec,A,$}



   \State $r\gets a\bmod b$
   \For{$  sentence \in sentenceBreak(W) $ }

      $ tokens \gets Tokenize(sentence) $
      \For{$ i in range(0, len(tokens) - 1) $}

        \State $a\gets b$
        \State $b\gets r$
        \State $r\gets a\bmod b$
     \EndFor \label{euclidendwhile}
   \EndFor
   \State \textbf{return} $b$\Comment{The gcd is b}
\EndProcedure
\end{algorithmic}
\end{algorithm}




System overview is this ....  \cite{nemanja-lasta},

==> texfiles/wiki-markup_results_annotated_text.tex <==


File Format Example:

% \begin{lstlisting}[language=json,firstnumber=1,breaklines=true,float=*,caption=JSON file format example.]]

